EqNIO: Subequivariant Neural Inertial Odometry

Neural networks are seeing rapid adoption in purely inertial odometry, where accelerometer and gyroscope measurements from commodity inertial measurement units (IMU) are used to regress displacements and associated uncertainties. They can learn informative displacement priors, which can be directly fused with the raw data with off-the-shelf non-linear filters. Nevertheless, these networks do not consider the physical roto-reflective symmetries inherent in IMU data, leading to the need to memorize the same priors for every possible motion direction, which hinders generalization. In this work, we characterize these symmetries and show that the IMU data and the resulting displacement and covariance transform equivariantly, when rotated around the gravity vector and reflected with respect to arbitrary planes parallel to gravity. We design a neural network that respects these symmetries by design through equivariant processing in three steps: First, it estimates an equivariant gravity-aligned frame from equivariant vectors and invariant scalars derived from IMU data, leveraging expressive linear and non-linear layers tailored to commute with the underlying symmetry transformation. We then map the IMU data into this frame, thereby achieving an invariant canonicalization that can be directly used with off-the-shelf inertial odometry networks. Finally, we map these network outputs back into the original frame, thereby obtaining equivariant covariances and displacements. We demonstrate the generality of our framework by applying it to the filter-based approach based on TLIO, and the end-to-end RONIN architecture, and show better performance on the TLIO, Aria, RIDI and OxIOD datasets than existing methods.

==> omega_symmetry_new.tex <==
% \begin{wrapfigure}{l}{0.5\linewidth}

%     \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=1.3in]{images/omega_symmetry_black.png}
%         \caption{}
%         \label{omega_symmetry_fig}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=1.3in]{images/preprocess_black_2.png}
%         \caption{}
%         \label{preprocess}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.55\textwidth}
%     %     \centering
%     %     \includegraphics[height=1in]{plot/nonlinear_new.png}
%     %     \caption{}
%     %     \label{nonlinear}
%     % \end{subfigure}
%     \caption{(a). Above: When $\omega$ (red) is reflected across a plane (blue), the corresponding rotations (black and gray arrowed arc ) are not correspondingly reflected. Bottom: To achieve the reflected rotations (black), $\omega$ should be reflected with a reversal of direction. (b). The rotation can be represented by $\omega$ or $v_1$(black) together with $v_2$ (blue). $v_1$ and $v_2$ represented the flow of the rotation. When the rotation is reflected, $v_1$ and $v_2$ are reflected. }
%     \vspace{-4mm}
% \end{wrapfigure}

%(c). Visualization of Nonlinearity.

% \begin{wrapfigure}{l}{0.5\linewidth}

%     % First row
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.45\linewidth]{plot/omega_symmetry_black.png}
%         \caption{}
%         \label{omega_symmetry_fig}
%     \end{subfigure}%
%     % \hfill
%     \vspace{-1mm} % Adjust space between rows if 
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.45\linewidth]{plot/preprocess_black_2.png}
%         \caption{}
%         \label{preprocess}
%     \end{subfigure}

%     \caption{(a). Above: When $\omega$ (red) is reflected across a plane (blue), the corresponding rotations (black and gray arrowed arc ) are not correspondingly reflected. Bottom: To achieve the reflected rotations (black), $\omega$ should be reflected with a reversal of direction. (b). The rotation can be represented by $\omega$ or $v_1$(black) together with $v_2$ (blue). $v_1$ and $v_2$ represented the flow of the rotation. When the rotation is reflected, $v_1$ and $v_2$ are reflected.}
%     \vspace{-2mm}
% \end{wrapfigure}

